VIRDO++: Real-World, Visuo-tactile Dynamics and Perception of Deformable Objects

Deformable objects manipulation can benefit from representations that seamlessly integrate vision and touch while handling occlusions. In this work, we present a novel approach for, and real-world demonstration of, multimodal visuo-tactile state-estimation and dynamics prediction for deformable objects. Our approach, VIRDO++, builds on recent progress in multimodal neural implicit representations for deformable object state-estimation [1] via a new formulation for deformation dynamics and a complementary state-estimation algorithm that (i) maintains a belief over deformations, and (ii) enables practical real-world application by removing the need for privileged contact information. In the context of two real-world robotic tasks, we show:(i) high-fidelity cross-modal state-estimation and prediction of deformable objects from partial visuo-tactile feedback, and (ii) generalization to unseen objects and contact formations.

==> text/01-introduction_old.tex <==
\section{Introduction}


% \textcolor{blue}{Dexterous manipulation of deformable objects is an important open problem in robotics~\cite{billard2019trends,yin2021modeling}. These objects are ubiquitous in our day-to-day lives and play a key role in many applications including manufacturing, in-home assistive care, surgery, and cooking, as shown in Fig.~\ref{fig:SDF}. Despite their prevalence and importance, deformable objects have received less attention than their rigid counterparts owing to their inherent complexities in modeling, perception, and controls \cite{yin2021modeling,sanchez2018robotic,arriola2020modeling,hou2019review}. To illustrate, the states of rigid bodies with known geometries can be succinctly represented with 6D pose and velocity. However, deformable objects have an infinite continuum of states and their representation and perception remains an open problem \cite{yin2021modeling}.}

% \textcolor{blue}{ In this paper, we present VIRDO -- an implicit, dense, cross modal, and continuous architecture that addresses these fundamental representation and perception challenges for the class of elastically deformable objects. The central feature of our method is learning deformation fields informed by cross modal visual and tactile cues of external contacts. We further contribute a dataset of elastically deformable objects with boundary conditions used to evaluate. This paper focuses on dense geometric representations because they can facilitate downstream tasks such as state-estimation from partial views and estimating dense correspondences, as we demonstrate, as well as bootstrapping keypoint/affordance learning.} Deformable tool manipulations are common in our day-to-day lives such as cooking, sweeping, and washing dishes. However, deformable objects are less explored in Robotics compare to their rigid counterparts. This is due to the difficulty at representing their infinite continuum of states and predicting/estimating the states under visual occlusion. 

Deformable objects are ubiquitous in our day to day lives. The cloths we wear, the food we eat, many of the tools we use, and our own biology are just a few examples. As such, robots must master dexterous manipulation of deformable objects. At the heart of this skill is mastery of the interplay between object geometry and force transmission, perceived by vision and touch. Deformable object manipulation is complicated by the complexity of this interplay (e.g., infinite dimensional state-space and nonlinearity) and the ensuing challenges in perception (e.g., partial observability and occlusion) and controls \cite{yin2021modeling,sanchez2018robotic,arriola2020modeling,hou2019review}. 

In this paper, we introduce \accro -- a novel multimodal, predictive, and continuous neural implicit representation -- to address modeling and perception challenges of deformable-elastic objects. Our representation models deformable objects as signed-distance and deformation vector fields built from partial point clouds and proprioceptive tactile feedback. These vector fields are indexed by a latent code that, when conditioned on robot actions, can also predict future deformations of objects. Our representation is capable of full 3D geometric shape estimation with dense correspondence in real-world robotic tasks, Fig. **teaser figure**. Our contributions are:

1. Multimodal neural implicit representation with action-conditioned dynamics to predict future deformations. This enables integration with downstream planning and control algorithms. To demonstrate the utility of the dynamics model, we introduce a state estimation algorithm based on the particle filter to maintain a belief distribution over object deformations.

2. Real-world demonstrations of \accro on two challenging tasks: scraping with a spatula and chain manipulation. We demonstrate both 3D geometry estimation in heavy occlusion and action-conditioned deformation/reaction wrench prediction. This is enabled by replacing contact formations with a novel \cntemb~that obfuscates the need for explicit contact patch information.

3. \todo{this contribution statement needs work}Zero-shot Generalization of \accro. Data is expensive in Robotics, and VIRDO's ability to generalize to different objects significantly reduces burden for data collection. 
% In detail, we propose a customization layer to represents unseen objects geometry and dynamics.  
% deformation field with pretrained VIRDO. Moreover, VIRDO learns to predict the unseen object's next state only given a few examples. In this way, VIRDO can be applied to many different off-the-shelf objects unseen during the training if they are in the same object class.

Our work extends \cite{young2022virdo} where a similar multimodal, continuous, and implicit representations was introduced with desirable features for robotic applications (e.g. dense geometric representations and state-estimation from partial views). Limitations of this work that we address here are that it is validated only in simulation and uses contact patches as one of its inputs (non-trivial to obtain in real robot tasks). Further, \cite{young2022virdo} represents objects in static scenes and does not handle the transition from deformation to deformation -- an important capability for many state-estimation and planning algorithm that requires an action-conditioned dynamics model. 

Implicit neural representations offer a number of advantages over their\todo{Do we need this? Or the rest of this paragraph}. These dense representations are also versatile for many downstream tasks including full 3D geometry estimation, goal-directed planning under occlusions, contact location estimation, and bootstrapping keypoint learning. 

% Main feature of \accro is using multi-modal encoder architectures to represent deformable objects states in low dimensional space and learn their dynamics from the learned latent spaces. Here, we adopt a continuous geometric representation because it provides versatility towards downstream tasks such as geometry estimation and goal-directed planning  


% \textbf{Why visio-tactile?}: Occlusions are common in tool use due to contact,  environment, and self-occlusion. Here, tactile, alongside with vision, helps reasoning about deformable objects' state or their deformations. With that in mind, \accro adopt both visual and tactile modalities in terms of representing dynamics of deformable objects. This multi-modal representation enables effective deformable object manipulation (ex. entangled strings) \cite{pecyna2022visual} and their state estimation. 






